Tensile quantum-to-classical transition of macroscopic entangled states under complete coarse-grained measurements

The macroscopic limit at which the quantum-to-classical transition occurs remains as one of the long-standing questions in the foundations of quantum theory. There are evidences that the macroscopic limit to which the quantumness of a system persists depends on the degree of interaction due to the measurement processes. For instance, with a system having a considerably large Hilbert space dimension, if the measurement is performed in such a way that the outcome of the measurement only reveals a coarse-grained version of the information about the individual level of the concerned system then the disturbance due to the measurement process can be considered to be infinitesimally small. Based on such coarse-grained measurement the dependence of Bell inequality violation on the degree of coarsening has already been investigated [Phys. Rev. Lett. 112, 010402 (2014)]. In this paper, we first capture the fact that when local-realism is taken to be the defining notion of classicality, the effect of the degree of coarsening on the downfall of quantumness of a macroscopic entangled state can be compensated by testing a Bell-inequality of a higher number of settings from a family of symmetric Bell-inequalities if the number of settings is odd. However, on the contrary, we show that such compensation can not be seen when we witness such quantum-to-classical transition using symmetric Bell inequalities having an even number of settings. Finally, complementing the above result, we show that when unsteerability is taken as the classicality, for both odd and even numbers of settings the degree of coarsening at which the quantum-to-classical transition occurs can be consistently pushed ahead by testing a linear steering inequality of a higher number of settings and observing its violation. We further extend our treatment for mixed macroscopic entangled states

==> name.tex <==
 The most well-known attempt to explain the quantum-to-classical transition is decoherence, which is the idea that interactions with the environment destroy quantum coherence, causing a quantum system to become classical \cite{decoher}.
But in more recent years, physicists have been investigating alternative explanations based on an observer's limited ability to control the precision of the measurements made on a system. The idea is that a system appears to exhibit quantum behavior when observed with very precise measurements will appear to behave classically if the measurements are too coarse or fuzzy. In such a scenario, the coarsening of measurements forces the quantum-to-classical transition .\\\\
The aforementioned explanations of the quantum-to-classical transition have emphasized the part that inefficiency in the final detection through coarsening i.e., measurement apparatus is unable to perfectly differentiate between elements of the measurement basis. Jeong \textit{et.al.} \cite{bar05} studied the phenomena of transition from quantum to classical behaviour  for macroscopic entangled states through the coarse-graining of measurement resolution and more importantly through coarse-graining of the measurement reference. The measurement reference play a major role in observing many quantum phenomena. In coarse graining of the measurement reference, the experimenter does not have complete control over the basis in which the measurement is being carried out. The authors demonstrated that, when subjected to these two different aspects of coarse-grained measurements; coarsening of the final measurement resolution
and that of the measurement reference lead to completely different results. Especially, when the measurement reference is coarsened, the quantum-to-classical transition is forced to occur, while it is not the case when the final projection is coarsened.\\\\
